Providing High and Controllable Performance in Multicore Systems Through Shared Resource Management

Multiple applications executing concurrently on a multicore system interfere with each other at different shared resources such as main memory and shared caches. Such inter-application interference, if uncontrolled, results in high system performance degradation and unpredictable application slowdowns. While previous work has proposed application-aware memory scheduling as a solution to mitigate inter-application interference and improve system performance, previously proposed memory scheduling techniques incur high hardware complexity and unfairly slowdown some applications. Furthermore, previously proposed memory-interference mitigation techniques are not designed to precisely control application performance. This dissertation seeks to achieve high and controllable performance in multicore systems by mitigating and quantifying the impact of shared resource interference. First, towards mitigating memory interference and achieving high performance, we propose the Blacklisting memory scheduler that achieves high performance and fairness at low complexity. Next, towards quantifying the impact of memory interference and achieving controllable performance in the presence of memory bandwidth interference, we propose the Memory Interference induced Slowdown Estimation (MISE) model. We propose and demonstrate two use cases that can leverage MISE to provide soft performance guarantees and high overall performance/fairness. Finally, we seek to quantify the impact of shared cache interference on application slowdowns, in addition to memory bandwidth interference. Towards this end, we propose the Application Slowdown Model (ASM). We propose and demonstrate several use cases of ASM that leverage it to provide soft performance guarantees and improve performance and fairness.

==> _ <==
\section{Evaluation}
\label{sec:blacklisting-evaluation}

We compare \bliss with five previously proposed memory schedulers,
FRFCFS, FRFCFS with a cap (FRFCFS-Cap)~\cite{stfm}, PARBS, ATLAS
and TCM.  FRFCFS-Cap is a modified version of FRFCFS that caps the
number of consecutive row-buffer hitting requests that can be
served from an application~\cite{stfm}.
Figure~\ref{fig:main-results} shows the average system performance
(weighted speedup and harmonic speedup) and unfairness (maximum
slowdown) across all our workloads. Figure~\ref{fig:pareto} shows
a pareto plot of weighted speedup and maximum slowdown. We draw
three major observations. First, \bliss achieves 5\% better
weighted speedup, 25\% lower maximum slowdown and 19\% better
harmonic speedup than the best performing previous scheduler
(in terms of weighted speedup), TCM, while reducing the critical path
and area by 79\% and 43\% respectively (as we will show in
Section~\ref{sec:blacklisting-complexity}). Therefore, we conclude that \bliss
achieves both high system performance and fairness, at low
hardware cost and complexity.

\begin{figure*}[ht!]
  \centering
  \begin{minipage}{0.32\textwidth}
    \centering
    \includegraphics[scale=0.21, angle=270]{blacklisting/plots/main_avg_unnorm_ws}
  \end{minipage}
  \begin{minipage}{0.32\textwidth}
    \centering
    \includegraphics[scale=0.21, angle=270]{blacklisting/plots/main_avg_unnorm_hs}
  \end{minipage}
  \begin{minipage}{0.32\textwidth}
    \centering
    \includegraphics[scale=0.21, angle=270]{blacklisting/plots/main_avg_unnorm_ms}
  \end{minipage}
  \caption{System performance and fairness of \bliss compared to previous schedulers}
  \label{fig:main-results}
\end{figure*}

Second, \bliss significantly outperforms all these five previous
schedulers in terms of system performance, however, it has 10\%
higher unfairness than PARBS, the previous scheduler with the
least unfairness. PARBS creates request batches containing the
oldest requests from each application. Older batches are
prioritized over newer batches. However, within each batch,
individual applications' requests are ranked and prioritized based
on memory intensity. PARBS aims to preserve fairness by batching
older requests, while still employing ranking within a batch to
prioritize low-memory-intensity applications. We observe that the
batching aspect of PARBS is quite effective in mitigating
unfairness, although it increases complexity. This unfairness
reduction also contributes to the high harmonic speedup of PARBS.
However, batching restricts the amount of request reordering that
can be achieved through ranking. Hence, low-memory-intensity
applications that would benefit from prioritization via aggressive
request reordering have lower performance. As a result, PARBS has
8\% lower weighted speedup than \bliss. Furthermore, PARBS has a
6.5x longer critical path and \httilde2x greater area than \bliss,
as we will show in Section~\ref{sec:blacklisting-complexity}. Therefore, we
conclude that \bliss achieves better system performance than
PARBS, at much lower hardware cost, while slightly trading off
fairness.


\begin{figure}[h]
    \centering
    \includegraphics[scale=0.3, angle=0]{blacklisting/plots/pareto.png}
    \caption{Pareto plot of system performance and fairness}
    \label{fig:pareto}
\end{figure}


Third, \bliss has 4\% higher unfairness than FRFCFS-Cap, but it
also 8\% higher performance than FRFCFS-Cap. FRFCFS-Cap has
higher fairness than \bliss since it restricts the length of
{\em only} the {\em ongoing} row hit streak, whereas blacklisting
an application can deprioritize the application {\em for a longer
time}, until the next clearing interval. As a result, FRFCFS-Cap
slows down high-row-buffer-locality applications to a lower degree
than \bliss. However, restricting \emph{only} the on-going streak
rather than blacklisting an interfering application for a longer
time causes more interference to other applications, degrading
system performance compared to \bliss. Furthermore, FRFCFS-Cap is
unable to mitigate interference due to applications with high
memory intensity yet low-row-buffer-locality, whereas \bliss is
effective in mitigating interference due to such applications as
well. Hence, we conclude that \bliss achieves higher performance
(weighted speedup) than FRFCFS-Cap, while slightly trading off
fairness.

\subsection{Analysis of Individual Workloads}
\label{sec:scurve-analysis}

In this section, we analyze the performance and fairness for
individual workloads, when employing different schedulers.
Figure~\ref{fig:scurve} shows the performance and fairness
normalized to the baseline FRFCFS scheduler for all our 80
workloads, for BLISS and previous schedulers, in the form of
S-curves~\cite{eaf}. The workloads are sorted based on the
performance improvement of BLISS. We draw three major
observations. First, BLISS achieves the best performance among all
previous schedulers for most of our workloads. For a few
workloads, ATLAS achieves higher performance, by virtue of always
prioritizing applications that receive low memory service.
However, always prioritizing applications that receive low memory
service can unfairly slow down applications with high memory
intensities, thereby degrading fairness significantly (as shown in
the maximum slowdown plot, Figure~\ref{fig:scurve} bottom).
Second, BLISS achieves significantly higher fairness than ATLAS
and TCM, the best-performing previous schedulers, while also
achieving higher performance than them and approaches the fairness
of the fairest previous schedulers, PARBS and FRFCFS-Cap. As
described in the analysis of average performance and fairness
results above, PARBS, by virtue of request batching and
FRFCFS-Cap, by virtue of restricting only the current row hit
streak achieve higher fairness (lower maximum slowdown) than BLISS
for a number of workloads. However, these schedulers achieve
higher fairness at the cost of lower system performance, as shown
in Figure~\ref{fig:scurve}. Third, for some workloads with very
high memory intensities, the default FRFCFS scheduler achieves the
best fairness. This is because memory bandwidth becomes a very
scarce resource when the memory intensity of a workload is very
high.  Hence, prioritizing row hits utilizes memory bandwidth
efficiently for such workloads, thereby resulting in higher
fairness. Based on these observations, we conclude that BLISS
achieves the best performance and a good trade-off between
fairness and performance for most of the workloads we examine.


\begin{figure*}[t!]
  \centering
  \begin{minipage}{0.48\textwidth}
    \centering
    \includegraphics[scale=0.3, angle=270]{blacklisting/plots/scurve_ws}
  \end{minipage}
  \begin{minipage}{0.48\textwidth}
    \centering
    \includegraphics[scale=0.3, angle=270]{blacklisting/plots/scurve_ms}
  \end{minipage}
  \caption{System performance and fairness for all workloads}
  \label{fig:scurve}
\end{figure*}

\subsection{Hardware Complexity}
\label{sec:blacklisting-complexity}

Figures~\ref{fig:crit-path-latency} and~\ref{fig:area} show the
critical path latency and area of five previous schedulers and
\bliss for a 24-core system for every memory channel. We draw two
major conclusions. First, previously proposed ranking-based
schedulers, PARBS/ATLAS/TCM, greatly increase the critical path
latency and area of the memory scheduler: by 11x/5.3x/8.1x and
2.4x/1.7x/1.8x respectively, compared to FRFCFS and FRFCFS-Cap,
whereas \bliss increases latency and area by only 1.7x and 3.2\%
over FRFCFS/FRFCFS-Cap.\footnote{The area numbers are for the
lowest value of critical path latency that the scheduler is able
to meet.} Second, PARBS, ATLAS and TCM cannot meet the stringent
worst-case timing requirements posed by the DDR3 and DDR4
standards~\cite{jedec-ddr3,jedec-ddr4}. In the case where every
request is a row-buffer hit, the memory controller would have to
schedule a request every read-to-read cycle time ($t_{CCD}$), the
minimum value of which is 4 cycles for both DDR3 and DDR4. TCM and
ATLAS can meet this worst-case timing only until DDR3-800
(read-to-read cycle time of 10 ns) and DDR3-1333 (read-to-read
cycle time of 6 ns) respectively, whereas \bliss can meet the
worst-case timing all the way down to the highest released
frequency for DDR4, DDR4-3200 (read-to-read time of 2.5 ns).
Hence, the high critical path latency of PARBS, ATLAS and TCM is a
serious impediment to their adoption in today's and future memory
interfaces. Techniques like pipelining could potentially be
employed to reduce the critical path latency of these previous
schedulers. However, the additional flops required for pipelining
would increase area, power and design effort significantly.
Therefore, we conclude that \bliss, with its greatly lower
complexity and cost as well as higher system performance and
competitive or better fairness, is a more effective alternative to
state-of-the-art application-aware memory schedulers.

\begin{figure}[ht]
  \centering
  \begin{minipage}{0.48\textwidth}
     \centering
     \includegraphics[scale=0.3, angle=270]{blacklisting/plots/latency}
     \caption{Critical path: \bliss vs. previous schedulers}
     \label{fig:crit-path-latency}
  \end{minipage}
  \begin{minipage}{0.48\textwidth}
%      \vspace{-1mm}
      \centering
      \includegraphics[scale=0.3, angle=270]{blacklisting/plots/area}
      \caption{Area: \bliss vs. previous schedulers}
      \label{fig:area}
  \end{minipage}
\end{figure}
\subsection{Analysis of Trade-offs Between Performance, Fairness and Complexity}
\label{sec:tradeoff-performance-fairness-complexity}

In the previous sections, we studied the performance, fairness and
complexity of different schedulers individually. In this section,
we will analyze the trade-offs between these metrics for
different schedulers. Figure~\ref{fig:perf-fairness-simplicity}
shows a three-dimensional radar plot with performance, fairness and
simplicity on three different axes. On the fairness axis, we plot
the negative of the maximum slowdown numbers, and on the simplicity axis, we
plot the negative of the critical path latency numbers. Hence, the ideal
scheduler would have high performance, fairness and simplicity, as
indicated by the encompassing, dashed black triangle. We draw three major conclusions
about the different schedulers we study. First,
application-unaware schedulers, such as FRFCFS and FRFCFS-Cap, are
simple. However, they have low performance and/or fairness. This
is because, as described in our performance analysis above, FRFCFS
allows long streaks of row hits from one application to cause
interference to other applications. FRFCFS-Cap attempts to tackle
this problem by restricting the length of current row hit streak.
While such a scheme improves fairness, it still does not improve
performance significantly. Second, application-aware schedulers,
such as PARBS, ATLAS and TCM, improve performance or fairness by
ranking based on applications' memory access characteristics.
However, they do so at the cost of increasing complexity (reducing
simplicity) significantly, since they employ a full ordered
ranking across all applications. Third, BLISS, achieves high
performance and fairness, while keeping the design simple, thereby
approaching the ideal scheduler design (i.e., leading to a
triangle that is closer to the ideal triangle). This is because BLISS
requires only simple hardware changes to the memory controller to
blacklist applications that have long streaks of requests served,
which effectively mitigates interference. Therefore, we conclude
that BLISS achieves the best trade-off between performance,
fairness and simplicity.

\begin{figure}[h]
    \centering
    \includegraphics[scale=0.4, angle=0]{blacklisting/plots/perf-fairness-simplicity-3d}
    \caption{Performance, fairness and simplicity trade-offs}
    \label{fig:perf-fairness-simplicity}
\end{figure}


\subsection{Understanding the Benefits of \bliss}
\label{sec:bliss-benefits}

We present the distribution of the number of consecutive requests
served (streaks) from individual applications to better understand
why \bliss effectively mitigates interference.
Figure~\ref{fig:streak_length} shows the distribution of requests
served across different streak lengths ranging from 1 to
16 for FRFCFS,
PARBS, TCM and \bliss for \emph{six representative applications
from the same 24-core workload}.\footnote{A value of 16 captures streak
lengths 16 and above.} The figure captions indicate the
memory intensity, in misses per kilo instruction (MPKI) and
row-buffer hit rate (RBH) of each application when it is run
alone. Figures~\ref{fig:libq},~\ref{fig:mcf} and~\ref{fig:lbm}
show the streak length distributions of applications that have a
tendency to cause interference ({\em libquantum}, {\em mcf} and
{\em lbm}). All these applications have high memory intensity
and/or high row-buffer locality.
Figures~\ref{fig:calculix},~\ref{fig:sphinx3} and~\ref{fig:cactus}
show applications that are vulnerable to interference ({\em
calculix}, {\em cactusADM} and {\em sphinx3}). These applications
have lower memory intensities and row-buffer localities, compared
to the interference-causing applications. We observe that \bliss
shifts the distribution of streak lengths towards the left for the
interference-causing applications, while it shifts the streak
length distribution to the right for the interference-prone
applications. Hence, \bliss breaks long streaks of consecutive
requests for interference-causing applications, while enabling
longer streaks for vulnerable applications. This enables such
vulnerable applications to make faster progress, thereby resulting
in better system performance and fairness. We have observed
similar results for most of our workloads.


\begin{figure*}[ht]
  \centering
  \begin{subfigure}[t]{0.32\textwidth}
    \centering
    \includegraphics[scale=0.2, angle=270]{blacklisting/plots/streaklength_libq}
    \caption{libquantum (MPKI: 52; RBH: 99\%)}
    \label{fig:libq}
  \end{subfigure}
  \begin{subfigure}[t]{0.32\textwidth}
    \centering
    \includegraphics[scale=0.2, angle=270]{blacklisting/plots/streaklength_mcf}
    \caption{mcf (MPKI: 146; RBH: 40\%)}
    \label{fig:mcf}
  \end{subfigure}
  \begin{subfigure}[t]{0.32\textwidth}
    \centering
    \includegraphics[scale=0.2, angle=270]{blacklisting/plots/streaklength_lbm}
    \caption{lbm (MPKI: 41; RBH: 89\%)}
    \label{fig:lbm}
  \end{subfigure}
  \begin{subfigure}[t]{0.32\textwidth}
    \centering
    \includegraphics[scale=0.2, angle=270]{blacklisting/plots/streaklength_calculix}
    \caption{calculix (MPKI: 0.1; RBH: 85\%)}
    \label{fig:calculix}
  \end{subfigure}
  \begin{subfigure}[t]{0.32\textwidth}
    \centering
    \includegraphics[scale=0.2, angle=270]{blacklisting/plots/streaklength_sphinx3}
    \caption{sphinx3 (MPKI: 24; RBH: 91\%)}
    \label{fig:sphinx3}
  \end{subfigure}
  \begin{subfigure}[t]{0.32\textwidth}
    \centering
    \includegraphics[scale=0.2, angle=270]{blacklisting/plots/streaklength_cactusADM}
    \caption{cactusADM (MPKI: 7; RBH: 49\%)}
    \label{fig:cactus}
  \end{subfigure}
  \caption{Distribution of streak lengths}
  \label{fig:streak_length}
\end{figure*}

\subsection{Average Request Latency}
\label{sec:average-request-latency}

In this section, we evaluate the average memory request latency
(from when a request is generated until when it is served)
metric and seek to understand its correlation with performance and
fairness. Figure~\ref{fig:latency} presents the average memory request
latency (from when the request is generated until when it is served)
for the five previously proposed memory schedulers and \bliss. Two
major observations are in order. First, FRFCFS has the lowest
average request latency among all the schedulers. This is
expected since FRFCFS maximizes DRAM throughput by prioritizing
row-buffer hits. Hence, the number of requests served is maximized
overall (across all applications). However, maximizing throughput
(i.e., minimizing overall average
request latency) degrades the performance of low-memory-intensity
applications, since these applications' requests are often delayed
behind row-buffer hits and older requests. This results in
degradation in system performance and fairness, as shown in
Figure~\ref{fig:main-results}. 

\begin{figure}[h!]
  \centering
  \includegraphics[scale=0.25, angle=270]{blacklisting/plots/main_avg_unnorm_avg_lat}
  \caption{The Average Request Latency Metric}
  \label{fig:latency}
\end{figure}

Second, ATLAS and TCM, memory schedulers that prioritize requests
of low-memory-intensity applications by employing a full ordered
ranking achieve relatively low average latency. This is because
these schedulers reduce the latency of serving requests from
latency-critical, low-memory-intensity applications significantly.
Furthermore, prioritizing low-memory-intensity applications'
requests does not increase the latency of high-memory-intensity
applications significantly. This is because high-memory-intensity
applications already have high memory access latencies (even when
run alone) due to queueing delays. Hence, average request latency does
not increase much from deprioritizing requests of such
applications. However, always prioritizing such latency-critical
applications results in lower memory throughput for
high-memory-intensity applications, resulting in unfair slowdowns
(as we show in Figure~\ref{fig:main-results}). Third, memory
schedulers that provide the best fairness, PARBS, FRFCFS-Cap and
\bliss have high average memory latencies. This is because these
schedulers, while employing techniques to prevent requests of
vulnerable applications with low memory intensity and low
row-buffer locality from being delayed, also avoid unfairly
delaying requests of high-memory-intensity applications. As a
result, they do not reduce the request service latency of
low-memory-intensity applications significantly, at the cost of
denying memory throughput to high-memory-intensity applications,
unlike ATLAS or TCM. Based on these observations, we conclude that while some
applications benefit from low memory access latencies, other
applications benefit more from higher memory throughput than lower
latency. Hence, average memory latency is {\em not} a suitable
metric to estimate system performance or fairness.

\subsection{Impact of Clearing the Blacklist Asynchronously}
\label{sec:blacklist-asynchronous-clearing}

The Blacklisting scheduler we have presented and evaluated so far
clears the blacklisting information periodically (every 10000
cycles in our evaluations so far), such that \emph{all}
applications are removed from the blacklist at the end of a
\textit{Clearing Interval}. In this section, we evaluate an
alternative design where an individual application is removed from
the blacklist \textit{Clearing Interval} cycles after it has been
blacklisted (independent of the other applications). In order to
implement this alternative design, each application would need an
additional counter to keep track of the number of remaining cycles
until the application would be removed from the blacklist. This
counter is set (to the \textit{Clearing Interval}) when an
application is blacklisted and is decremented every cycle until it
becomes zero. When it becomes zero, the corresponding application
is removed from the blacklist. We use a \textit{Clearing Interval}
of 10000 cycles for this alternative design as well.     

Table~\ref{tab:individual-clearing} shows the system performance
and fairness of the original BLISS design (BLISS) and the
alternative design in which individual applications are removed
from the blacklist asynchronously (BLISS-Individual-Clearing). As
can be seen, the performance and fairness of the two designs are
similar. Furthermore, the first design (BLISS) is simpler since it
does not need to maintain an additional counter for each
application. We conclude that the original BLISS design is
more efficient, in terms of performance, fairness and complexity.

\begin{table}[h!]
  \centering
  \input{blacklisting/tables/individual-clearing}
  \caption{Clearing the blacklist asynchronously}
  \label{tab:individual-clearing}
\end{table}

\subsection{Comparison with TCM's Clustering Mechanism}
\label{sec:tcm-clustering}

Figure~\ref{fig:tcm-no-ranking} shows the system performance and
fairness of \bliss, TCM and TCM's clustering mechanism
(TCM-Cluster). TCM-Cluster is a modified version of TCM that
performs clustering, but does not rank applications within each
cluster. We draw two major conclusions. First, TCM-Cluster has
similar system performance as \bliss, since both \bliss and
TCM-Cluster prioritize vulnerable applications by separating them
into a group and prioritizing that group rather than ranking
individual applications. Second, TCM-Cluster has significantly
higher unfairness compared to \bliss. This is because TCM-Cluster
always deprioritizes high-memory-intensity applications,
regardless of whether or not they are causing interference (as
described in Observation 2 in Section~\ref{sec:blacklisting-observations}).
\bliss, on the other hand, observes an application at fine time
granularities, independently at every memory channel and
blacklists an application at a channel {\em only when} it is
generating a number of consecutive requests (i.e., potentially
causing interference to other applications).

\begin{figure*}[hbt!]
  \centering
  \begin{minipage}{0.31\textwidth}
    \centering
    \includegraphics[scale=0.2, angle=270]{blacklisting/plots/tcm_no_rank_comparison_ws}
  \end{minipage}
  \begin{minipage}{0.31\textwidth}
    \centering
    \includegraphics[scale=0.2, angle=270]{blacklisting/plots/tcm_no_rank_comparison_hs}
  \end{minipage} 
  \begin{minipage}{0.31\textwidth}
    \centering
    \includegraphics[scale=0.2, angle=270]{blacklisting/plots/tcm_no_rank_comparison_ms}
  \end{minipage} 
  \caption{Comparison with TCM's clustering mechanism}
  \label{fig:tcm-no-ranking}
\end{figure*}


\subsection{Evaluation of Row Hit Based Blacklisting}
\label{sec:blacklisting-frfcfs-cap}

\bliss, by virtue of restricting the number of consecutive
requests that are served from an application, attempts to mitigate
the interference caused by both high-memory-intensity and high-
row-buffer-locality applications. In this section, we attempt to
isolate the benefits from restricting consecutive row-buffer
hitting requests vs. non-row-buffer hitting requests. To this end,
we evaluate the performance and fairness benefits of a mechanism
that places an application in the blacklist when a certain number
of row-buffer hitting requests (\textrm{N}) to the same row have
been served for an application (we call this
FRFCFS-Cap-Blacklisting as the scheduler essentially is FRFCFS-Cap
with blacklisting). We use an \textrm{N} value of 4 in our
evaluations.

\begin{sloppypar}
Figure~\ref{fig:frfcfs-cap-blacklisting} compares the system
performance and fairness of \bliss with FRFCFS-Cap-Blacklisting.
We make three major observations. First, FRFCFS-Cap-Blacklisting
has similar system performance as \bliss.  On further analysis of
individual workloads, we find that FRFCFS-Cap-Blacklisting
blacklists only applications with high row-buffer locality,
causing requests of non-blacklisted high-memory-intensity
applications to interfere with requests of low-memory-intensity
applications. However, the performance impact of this interference
is offset by the performance improvement of high-memory-intensity
applications that are not blacklisted. Second,
FRFCFS-Cap-Blacklisting has higher unfairness (higher maximum
slowdown and lower harmonic speedup) than \bliss. This is because
the high-memory-intensity applications that are not blacklisted
are prioritized over the blacklisted high-row-buffer-locality
applications, thereby interfering with and slowing down the high-
row-buffer-locality applications significantly. Third,
FRFCFS-Cap-Blacklisting requires a per-bank counter to count and
cap the number of row-buffer hits, whereas \bliss needs only one
counter per-channel to count the number of consecutive requests
from the same application. Therefore, we conclude that \bliss is
more effective in mitigating unfairness while incurring lower
hardware cost, than the FRFCFS-Cap-Blacklisting scheduler that we
build combining principles from FRFCFS-Cap and BLISS.
\end{sloppypar}

\begin{figure*}[ht!]
  \centering
  \begin{minipage}{0.31\textwidth}
    \centering
    \includegraphics[scale=0.2, angle=270]{blacklisting/plots/frfcfs_cap_blacklisting_ws}
  \end{minipage}
  \begin{minipage}{0.31\textwidth}
    \centering
    \includegraphics[scale=0.2, angle=270]{blacklisting/plots/frfcfs_cap_blacklisting_hs}
  \end{minipage}
  \begin{minipage}{0.31\textwidth}
    \centering
    \includegraphics[scale=0.2, angle=270]{blacklisting/plots/frfcfs_cap_blacklisting_ms}
  \end{minipage}
  \caption{Comparison with FRFCFS-Cap combined with blacklisting}
  \label{fig:frfcfs-cap-blacklisting}
\end{figure*}

\subsection{Comparison with Criticality-Aware Scheduling}

We compare the system performance and fairness of \bliss with
those of criticality-aware memory
schedulers~\cite{crit-scheduling-cornell}. The basic idea behind
criticality-aware memory scheduling is to prioritize memory
requests from load instructions that have stalled the instruction
window for long periods of time in the past. Ghose et
al.~\cite{crit-scheduling-cornell} evaluate prioritizing load
requests based on both maximum stall time (Crit-MaxStall) and
total stall time (Crit-TotalStall) caused by load instructions in
the past. Figure~\ref{fig:crit-comparison} shows the system
performance and fairness of \bliss and the criticality-aware
scheduling mechanisms, normalized to FRFCFS, across 40 workloads.
Two observations are in order. First, \bliss significantly
outperforms criticality-aware scheduling mechanisms in terms of
both system performance and fairness. This is because the
criticality-aware scheduling mechanisms unfairly deprioritize and
slow down low-memory-intensity applications that inherently
generate fewer requests, since stall times tend to be low for such
applications. Second, criticality-aware scheduling incurs hardware
cost to prioritize requests with higher stall times. Specifically,
the number of bits to represent stall times is on the order of
12-14, as described in~\cite{crit-scheduling-cornell}. Hence, the
logic for comparing stall times and prioritizing requests with
higher stall times would incur even higher cost than
per-application ranking mechanisms where the number of bits to
represent a core's rank grows only as as $log_2 Number Of Cores$
(e.g. 5 bits for a 32-core system). Therefore, we conclude that
\bliss achieves significantly better system performance and
fairness, while incurring lower hardware cost.

\begin{figure}[ht!]
  \vspace{-4mm}
  \centering
  \begin{minipage}{0.45\textwidth}
    \centering
    \includegraphics[scale=0.25, angle=270]{blacklisting/plots/crit_comparison_ws}
  \end{minipage}
  \begin{minipage}{0.45\textwidth}
   \centering
   \includegraphics[scale=0.25, angle=270]{blacklisting/plots/crit_comparison_ms}
  \end{minipage}
  \vspace{-2mm}
  \caption{Comparison with criticality-aware scheduling}
  \label{fig:crit-comparison}
  \vspace{-3.5mm}
\end{figure}

\subsection{Effect of Workload Memory Intensity and Row-buffer Locality}

In this section, we study the impact of workload memory intensity
and row-buffer locality on performance and fairness of \bliss and
five previous schedulers.

\noindent\textbf{Workload Memory Intensity.}
Figure~\ref{fig:intensity-results} shows system performance and
fairness for workloads with different memory intensities,
classified into different categories based on the fraction of
high-memory-intensity applications in a workload.\footnote{We
classify applications with MPKI less than 5 as
low-memory-intensity and the rest as high-memory-intensity.}  We
draw three major conclusions.  First, \bliss outperforms previous
memory schedulers in terms of system performance across all
intensity categories. Second, the system performance benefits of
\bliss increase with workload memory intensity. This is because as
the number of high-memory-intensity applications in a workload
increases, ranking individual applications, as done by previous
schedulers, causes more unfairness and degrades system
performance. Third, \bliss achieves significantly lower unfairness
than previous memory schedulers, except FRFCFS-Cap and PARBS,
across all intensity categories. Therefore, we conclude that
\bliss is effective in mitigating interference and improving
system performance and fairness across workloads with different
compositions of high- and low-memory-intensity applications.

\begin{figure}[h!]
  \centering
  \begin{minipage}{0.45\textwidth}
    \centering
    \includegraphics[scale=0.25, angle=270]{blacklisting/plots/intensity_results_ws}
  \end{minipage}
  \begin{minipage}{0.45\textwidth}  
    \centering
    \includegraphics[scale=0.25, angle=270]{blacklisting/plots/intensity_results_ms}
  \end{minipage}
  \caption{Sensitivity to workload memory intensity}
  \label{fig:intensity-results}
\end{figure}
\noindent\textbf{Workload Row-buffer Locality.}
Figure~\ref{fig:row-locality-results} shows the system performance
and fairness of five previous schedulers and BLISS when the number
of high row-buffer locality applications in a workload is
varied.\footnote{We classify an application as having high
row-buffer locality if its row-buffer hit rate is greater than
90\%.} We draw three observations. First, BLISS achieves the best
performance and close to the best fairness in most row-buffer
locality categories. Second, BLISS' performance and fairness
benefits over baseline FRFCFS increase as the number of
high-row-buffer-locality applications in a workload increases.
As the number of high-row-buffer-locality
applications in a workload increases, there is more interference to
the low-row-buffer-locality applications that are vulnerable.
Hence, there is more opportunity for BLISS to mitigate this
interference and improve performance and fairness. Third, when all
applications in a workload have high row-buffer locality (100\%),
the performance and fairness improvements of BLISS over baseline
FRFCFS are a bit lower than the other categories. This is because,
when all applications have high row-buffer locality, they each hog
the row-buffer in turn and are not as susceptible to interference
as the other categories in which there are vulnerable
low-row-buffer-locality applications. However, the
performance/fairness benefits of BLISS are still significant since BLISS is
effective in regulating how the row-buffer is shared among 
different applications. Overall, we conclude that BLISS is
effective in achieving high performance and fairness across
workloads with different compositions of high- and low-row-buffer-locality
applications.

\begin{figure}[h!]
  \centering
  \begin{minipage}{0.45\textwidth}
    \centering
    \includegraphics[scale=0.25, angle=270]{blacklisting/plots/rowlocality_sweep_ws}
  \end{minipage}
  \begin{minipage}{0.45\textwidth}  
    \centering
    \includegraphics[scale=0.25, angle=270]{blacklisting/plots/rowlocality_sweep_ms}
  \end{minipage}
  \caption{Sensitivity to row-buffer locality}
  \label{fig:row-locality-results}
\end{figure}


\subsection{Sensitivity to System Parameters}
\label{sec:sensitivity-system}

\noindent\textbf{Core and channel count.}
Figures~\ref{fig:sensitivity-num-cores}
and~\ref{fig:sensitivity-num-channels} show the system performance
and fairness of FRFCFS, PARBS, TCM and \bliss for different core
counts (when the channel count is 4) and different channel counts
(when the core count is 24), across 40 workloads for each
core/channel count. The numbers over the bars indicate percentage
increase or decrease compared to FRFCFS. We did not optimize the
parameters of different schedulers for each configuration as this
requires months of simulation time. We draw three major
conclusions. First, the absolute values of weighted speedup
increases with increasing core/channel count, whereas the absolute
values of maximum slowdown increase/decrease with increasing
core/channel count respectively, as expected. 
\begin{figure}[h!]
    \centering
    \begin{minipage}{0.45\textwidth}
       \centering
       \includegraphics[scale=0.25, angle=270]{blacklisting/plots/sensitivity_core_ws}
    \end{minipage}
    \begin{minipage}{0.45\textwidth}
       \centering
        \includegraphics[scale=0.25, angle=270]{blacklisting/plots/sensitivity_core_ms}
    \end{minipage}
    \caption{Sensitivity to number of cores}
    \label{fig:sensitivity-num-cores}
\end{figure}
\begin{figure}[h!]
    \centering
    \begin{minipage}{0.45\textwidth}
       \centering
       \includegraphics[scale=0.25, angle=270]{blacklisting/plots/sensitivity_channel_ws}
    \end{minipage}
    \begin{minipage}{0.45\textwidth}
       \centering
        \includegraphics[scale=0.25, angle=270]{blacklisting/plots/sensitivity_channel_ms}
    \end{minipage}
    \caption{Sensitivity to number of channels}
    \label{fig:sensitivity-num-channels}
\end{figure}
\noindent
Second, \bliss achieves higher system performance and lower
unfairness than all the other scheduling policies (except PARBS,
in terms of fairness) similar to our results on the 24-core,
4-channel system, by virtue of its effective interference
mitigation. The only anomaly is that TCM has marginally higher
weighted speedup than \bliss for the 64-core system. However, this
increase comes at the cost of significant increase in unfairness.
Third, \bliss' system performance benefit (as indicated by the
percentages on top of bars, over FRFCFS) increases when the system
becomes more bandwidth constrained, i.e., high core counts and low
channel counts. As contention increases in the system, \bliss has
greater opportunity to mitigate it.\footnote{Fairness benefits
reduce at very high core counts and very low channel counts, since
memory bandwidth becomes highly saturated.}

\noindent\textbf{Cache size.}
Figure~\ref{fig:sensitivity-cache-size} shows the system
performance and fairness for five previous schedulers and BLISS
with different last level cache sizes (private to each core).  

\begin{figure}[ht!]
    \centering
    \begin{minipage}{0.45\textwidth}
       \centering
       \includegraphics[scale=0.25, angle=270]{blacklisting/plots/sensitivity_cache_size_ws}
    \end{minipage}
    \begin{minipage}{0.45\textwidth}
       \centering
        \includegraphics[scale=0.25, angle=270]{blacklisting/plots/sensitivity_cache_size_ms}
    \end{minipage}
    \caption{Sensitivity to cache size}
    \label{fig:sensitivity-cache-size}
\end{figure}

We make two observations. First, the absolute values of weighted
speedup increase and maximum slowdown decrease, as the cache size
becomes larger for all schedulers, as expected. This is because
contention for memory bandwidth reduces with increasing cache
capacity, improving performance and fairness. Second, across all
the cache capacity points we evaluate, BLISS achieves significant
performance and fairness benefits over the best-performing
previous schedulers, while approaching close to the fairness of
the fairest previous schedulers.

\noindent\textbf{Shared Caches.} Figure~\ref{fig:shared-cache}
shows system performance and fairness with a 32 MB shared cache
(instead of the 512 KB per core private caches used in our other
experiments). \bliss achieves 5\%/24\% better performance/fairness
compared to TCM, demonstrating that \bliss is effective in
mitigating memory interference in the presence of large shared caches as
well.

\begin{figure}[ht!]
    \centering
    \begin{minipage}{0.45\textwidth}
       \centering
       \includegraphics[scale=0.25, angle=270]{blacklisting/plots/shared-cache-ws}
    \end{minipage}
    \begin{minipage}{0.45\textwidth}
       \centering
        \includegraphics[scale=0.25, angle=270]{blacklisting/plots/shared-cache-ms}
    \end{minipage}
    \caption{Performance and fairness with a shared cache}
    \label{fig:shared-cache}
\end{figure}

\subsection{Sensitivity to Algorithm Parameters}
\label{sec:sensitivity-algorithm}

Tables~\ref{tab:sensitivity-ws} and \ref{tab:sensitivity-ms} show
the system performance and fairness respectively of \bliss for
different values of the \textit{Blacklisting Threshold} and
\textit{Clearing Interval}. Three major conclusions are in order.
First, a \textit{Clearing Interval} of 10000 cycles provides a
good balance between performance and fairness. If the blacklist is
cleared too frequently (1000 cycles), interference-causing
applications are not deprioritized for long enough, resulting in
low system performance. In contrast, if the blacklist is cleared
too infrequently, interference-causing applications are
deprioritized for too long, resulting in high unfairness. Second,
a \textit{Blacklisting Threshold} of 4 provides a good balance
between performance and fairness. When \textit{Blacklisting
Threshold} is very small, applications are blacklisted as soon as
they have very few requests served, resulting in poor interference
mitigation as too many applications are blacklisted. On the other
hand, when \textit{Blacklisting Threshold} is large, low- and
high-memory-intensity applications are not segregated effectively,
leading to high unfairness. 


\begin{table}[ht]
  \centering
  \input{blacklisting/tables/sensitivity-ws}
  \caption{Performance sensitivity to threshold and interval}
  \label{tab:sensitivity-ws}
\end{table}


\begin{table}[ht]
  \centering
  \input{blacklisting/tables/sensitivity-ms}
  \caption{Unfairness sensitivity to threshold and interval}
  \label{tab:sensitivity-ms}
\end{table}

\subsection{Interleaving and Scheduling Interaction}
\label{sec:interleaving-interaction}

In this section, we study the impact of the address interleaving
policy on the performance and fairness of different schedulers.
Our analysis so far has assumed a row-interleaved policy, where
data is distributed across channels, banks and rows at the
granularity of a row. This policy optimizes for row-buffer
locality by mapping a consecutive row of data to the same channel,
bank, rank. In this section, we will consider two other
interleaving policies, cache block interleaving and sub-row
interleaving.

\noindent\textbf{Interaction with cache block interleaving.} In a
cache-block-interleaved system, data is striped across channels,
banks and ranks at the granularity of a cache block.  Such a
policy optimizes for bank level parallelism, by distributing data
at a small (cache block) granularity across channels, banks and
ranks. 

Figure~\ref{fig:cacheblockint-interaction} shows the system
performance and fairness of FRFCFS with row interleaving
(FRFCFS-Row), as a comparison point, five previous schedulers, and
BLISS with cache block interleaving. We draw three observations.
First, system performance and fairness of the baseline FRFCFS
scheduler improve significantly with cache block interleaving,
compared to with row interleaving. This is because cache block
interleaving enables more requests to be served in parallel at the
different channels and banks, by distributing data across channels
and banks at the small granularity of a cache block. Hence, most
applications, and particularly, applications that do not have very
high row-buffer locality benefit from cache block interleaving.

\begin{figure}[ht]
  \centering
  \begin{minipage}{0.45\textwidth}
    \centering
    \includegraphics[scale=0.25, angle=270]{blacklisting/plots/cacheblockint-interaction-ws}
  \end{minipage}
  \begin{minipage}{0.45\textwidth}
    \centering
    \includegraphics[scale=0.25, angle=270]{blacklisting/plots/cacheblockint-interaction-ms}
  \end{minipage}
  \caption{Scheduling and cache block interleaving}
  \label{fig:cacheblockint-interaction}
\end{figure}

Second, as expected, application-aware schedulers such as ATLAS
and TCM achieve the best performance among previous schedulers, by
means of prioritizing requests of applications with low memory
intensities. However, PARBS and FRFCFS-Cap do not improve fairness
over the baseline, in contrast to our results with row
interleaving. This is because cache block interleaving already
attempts to provide fairness by increasing the parallelism in the
system and enabling more requests from across different
applications to be served in parallel, thereby reducing unfair
applications slowdowns. More specifically, requests that would
be row-buffer hits to the same bank, with row interleaving,
are now distributed across multiple channels and banks, with cache
block interleaving. Hence, applications' propensity to cause
interference reduces, providing lower scope for request capping
based schedulers such as FRFCFS-Cap and PARBS to mitigate
interference.  Third, BLISS achieves within 1.3\% of the
performance of the best performing previous scheduler (ATLAS),
while achieving 6.2\% better fairness than the fairest previous
scheduler (PARBS). BLISS effectively mitigates interference by
regulating the number of consecutive requests served from
high-memory-intensity applications that generate a large number of
requests, thereby achieving high performance and fairness.\\
\noindent\textbf{Interaction with sub-row interleaving.} While
memory scheduling has been a prevalent approach to mitigate memory
interference, previous work has also proposed other solutions, as
we describe in Section~\ref{chap:background}. One such previous
work by Kaseridis et al.~\cite{mop} proposes {\em minimalist open
page}, an interleaving policy that distributes data across
channels, ranks and banks at the granularity of a sub-row (partial
row), rather than an entire row, exploiting both row-buffer
locality and bank-level parallelism. We examine BLISS' interaction
with such a sub-row interleaving policy.

Figure~\ref{fig:subrowint-interaction} shows the system
performance and fairness of FRFCFS with row interleaving
(FRFCFS-Row), FRFCFS with cache block interleaving (FRFCFS-Block)
and five previously proposed schedulers and \bliss, with sub-row
interleaving (when data is striped across channels, ranks and
banks at the granularity of four cache blocks). Three observations
are in order. First, sub-row interleaving provides significant
benefits over row interleaving, as can be observed for FRFCFS (and
other scheduling policies by comparing with
Figure~\ref{fig:main-results}). This is because sub-row
interleaving enables applications to exploit both row-buffer
locality and bank-level parallelism, unlike row interleaving that
is mainly focused on exploiting row-buffer locality. Second,
sub-row interleaving achieves similar performance and fairness as
cache block interleaving. We observe that this is because cache
block interleaving enables applications to exploit parallelism
effectively, which makes up for the lost row-buffer locality from
distributing data at the granularity of a cache block across all
channels and banks. Third, BLISS achieves close to the performance
(within 1.5\%) of the best performing previous scheduler (TCM),
while reducing unfairness significantly and approaching the
fairness of the fairest previous schedulers. One thing to note is
that BLISS has higher unfairness than FRFCFS, when a
sub-row-interleaved policy is employed. This is because the
capping decisions from sub-row interleaving and BLISS could
collectively restrict high-row-buffer locality applications to a
large degree, thereby slowing them down and causing higher
unfairness. Co-design of the scheduling and interleaving policies
to achieve different goals such as performance/fairness is an
important area of future research. We conclude that a \bliss-like
scheduler, with its high performance and low complexity is a
significantly better alternative to schedulers such as ATLAS/TCM
in the pursuit of such scheduling-interleaving policy co-design.

\begin{figure}[h]
  \centering
  \begin{minipage}{0.45\textwidth}
    \centering
    \includegraphics[scale=0.25, angle=270]{blacklisting/plots/subrowint-interaction-ws}
  \end{minipage}
%  \vspace{-2mm}
  \begin{minipage}{0.45\textwidth}
    \centering
    \includegraphics[scale=0.25, angle=270]{blacklisting/plots/subrowint-interaction-ms}
  \end{minipage}
  \caption{Scheduling and sub-row interleaving}
  \label{fig:subrowint-interaction}
\end{figure}



==> applications-asm/applications.tex <==
\section{Leveraging ASM's Slowdown Estimates}
\label{sec:applications}

\asm's slowdown estimates can be leveraged to build various
slowdown-aware mechanisms to improve performance, fairness, and
provide slowdown guarantees. In this section, we present
five such use cases of \asm.



%and evaluate two of them: 1)~a
%slowdown-aware cache partitioning mechanism, and 2)~a
%slowdown-aware memory bandwidth partitioning mechanism in
%detail.\footnote{For these two mechanisms, we use a quantum length
%of 1,000,000 cycles.}


%% \asm's slowdown estimates can be leveraged to build various
%% schemes with the goals of improving performance, fairness and
%% providing performance predictability. In this section, we propose
%% two such mechanisms, 1) a scheme that partitions the shared cache
%% capacity among applications in a slowdown-aware manner, 2) a
%% scheme that partitions memory bandwidth among applications in a
%% slowdown-aware manner.



%% Slowdown estimates from the ASM model can be leveraged to build
%% various schemes with the goals of improving performance, fairness
%% and providing performance predictability. In this section, we
%% present and evaluate two such schemes. First, we present a scheme
%% that leverages slowdown estimates from the ASM model to partition
%% the shared cache capacity among applications. Second, we will
%% present a scheme that partitions memory bandwidth among
%% applications.

\input{sections/application-cache.tex}
\input{sections/application-memory.tex}
\input{sections/application-performance-guarantees.tex}
\input{sections/application-fair-billing.tex}
\input{sections/application-migration-admission-control.tex}


%In this section, we evaluate the fairness and performance benefits of combining
%ASM-Cache and ASM-Mem, in comparison with combining previous
%scheduling policies with utility-based cache partitioning (UCP).
%Figure~\ref{fig:cachepart-bwpart-results} compares ASM-Cache-Mem that
%combines ASM-Cache and ASM-Mem with TCM and PARBS combined with UCP.
%We draw two observations. First, ASM-Cache-Mem significantly reduces
%unfairness compared to TCM+UCP, PARBS+UCP and UCP, while achieving comparable
%performance. Second, ASM-Cache-Mem also achieves significant unfairness
%reduction compared to previous schemes that manage cache, memory bandwidth
%interference alone such as UCP, TCM and PARBS. These benefits come from the
%ability to partition cache capacity and memory bandwidth among applications
%based directly on slowdown estimates from ASM, rather than employing proxies
%such as miss count, memory intensity. The benefits over FST come
%from the fact that FST's slowdown estimates are not very accurate,
%especially as the core count increases. Therefore, we conclude that ASM is an
%effective substrate on which cache management, memory management, combined
%cache/memory management schemes can be built effectively, achieving high
%fairness and performance. 
%
%\begin{figure}[h!]
%  \vspace{-1mm}
%  \centering
%  \begin{minipage}{0.22\textwidth}
%    \centering
%    \includegraphics[scale=0.17, angle=270]{plots/cachepart_bwpart_hs}
%  \end{minipage}
%  \hspace{2mm}
%  \begin{minipage}{0.22\textwidth}  
%    \centering
%    \includegraphics[scale=0.17, angle=270]{plots/cachepart_bwpart_ms}
%  \end{minipage}
%  \caption{ASM-Cache-Mem: Performance and fairness}
%  \label{fig:cachepart-bwpart-results}
%\end{figure}





==> applications-asm/tables/methodology.tex <==
\begin{table}[h!]
%\vspace{-3mm}
  \begin{small}
    \centering
    \begin{tabular}{p{0.28\linewidth}p{0.62\linewidth}}
      \toprule
      \multirow{2}{*}{\textbf{Processor}} &  4-16 cores, 5.3GHz, 3-wide issue, 128-entry instruction window\\
      \midrule
      \multirow{2}{*}{\textbf{L1 cache}} &  64KB, private, 4-way associative, LRU, line size =
      64B, latency = 1 cycle\\
      \midrule
      \multirow{2}{*}{\textbf{Last-level cache}} & 1MB-4MB, shared, 16-way associative, LRU,
      line size = 64B, latency = 20 cycles\\
      \midrule
      \multirow{2}{*}{\textbf{Memory controller}} &  128-entry request buffer per
      controller, FR-FCFS~\cite{frfcfs} scheduling policy\\
      \midrule
      \multirow{3}{*}{\textbf{Main Memory}} & DDR3-1333 (10-10-10)~\cite{micron}, 1-4 channels,
      \mbox{1 rank/channel}, 8 banks/rank, 8KB rows\\
      \bottomrule
    \end{tabular}
    \vspace{-1mm}
    \caption{Configuration of the simulated system}
    \label{tab:meth}
  \end{small}
\vspace{-2mm}
\end{table}



==> applications-asm/tables/sensitivity-epoch-quantum.tex <==
\begin{tabular}{cccccc}
  \toprule
  \backslashbox{Quantum Length}{Epoch Length} & 10000 & 50000 & 100000\\
  \toprule
  1000000 & 12\% & 14\% & 16.6\% \\
  \midrule
  5000000 & 9.9\% & 10.6\%  & 11.5\%\\
  \midrule
  10000000 & 9.2\% & 9.9\% & 10.5\%\\
  \bottomrule
\end{tabular}



==> applications-mise-model/tables/interval-epoch-sensitivity.tex <==
\footnotesize{
%\begin{tabular}{|c|c|c|c|}
%  \hline
%   Epoch Length & 1000 & 10000 & 100000\\
%  \hline
%   Avg. Error (in \%) & 9.1 & 8.1 & 11.2\\
%  \hline
%  \hline
%  Interval Length & 1 mil & 5 mil & 10 mil\\
%  \hline
%  Avg. Error (in \%) & 64.1 & 8.1 & 9.6 \\
%  \hline
%\end{tabular}

\begin{tabular}{|c|c|c|c|c|c|}
  \hline
  \backslashbox{Epoch\\Length}{Interval\\Length} & 1 mil. & 5 mil. & 10 mil. & 25 mil. & 50 mil.\\
  \hline
  1000 & 65.1\% & 9.1\% & 11.5\% & 10.7\% & 8.2\%\\
  \hline
  10000 & 64.1\% & 8.1\% & 9.6\% & 8.6\% & 8.5\%\\
  \hline
  100000 & 64.3\% & 11.2\% & 9.1\% & 8.9\% & 9\%\\
  \hline
  1000000 & 64.5\% & 31.3\% & 14.8\% & 14.9\% & 11.7\%\\
  \hline
\end{tabular}
}


==> applications-mise-model/tables/methodology.tex <==
\begin{table}[h!]
\begin{footnotesize}
  \centering
    \begin{tabular}{ll}
        \toprule
Processor           &  4-16 cores, 5.3GHz, 3-wide issue,\\ & 8 MSHRs, 128-entry instruction window     \\
        \cmidrule(rl){1-2}
Last-level cache    &  64B cache-line, 16-way associative,\\ & 512kB private cache-slice per core     \\
        \cmidrule(rl){1-2} Memory controller   &  64/64-entry read/write request queues per controller   \\
        \cmidrule(rl){1-2}
\multirow{2}[2]{*}{\centering Memory}              &  Timing: DDR3-1066 (8-8-8)~\cite{micron} \\
 & Organization: 1 channel, 1
 rank-per-channel,\\ & 8 banks-per-rank, 8 KB row-buffer \\ 
        \bottomrule
    \end{tabular}%
  \caption{Configuration of the simulated system}
  \label{tab:meth}%
\end{footnotesize}%
\end{table}%


==> applications-mise-model/tables/slowdown-errors.tex <==
\footnotesize{
\begin{tabular}{|c|c|c||c|c|c|}
  \hline
  \textbf{Benchmark} & \textbf{STFM} & \textbf{\miiseabb\xspace} & \textbf{Benchmark} & \textbf{STFM} & \textbf{\miiseabb\xspace}\\
%  \textbf{Benchmark} & \textbf{STFM - Avg. Error (in \%)} & \textbf{\miiseabb\xspace - Avg. Error (in \%)} & \textbf{Benchmark} & \textbf{STFM - Avg. Error (in \%)} & \textbf{\miiseabb\xspace  - Avg. Error (in \%)}\\
  \hline
  453.povray & 56.3 & 0.1 & 473.astar & 12.3 & 8.1\\
  \hline
  454.calculix & 43.5 & 1.3 & 456.hmmer & 17.9 & 8.1\\
  \hline
  400.perlbench	& 26.8 & 1.6 & 464.h264ref & 13.7 & 8.3\\
  \hline
  447.dealII & 37.5 & 2.4 & 401.bzip2 &	28.3 & 8.5\\
  \hline
  436.cactusADM	& 18.4 & 2.6 & 458.sjeng & 21.3 & 8.8\\
  \hline
  450.soplex & 29.8 & 3.5 & 433.milc & 26.4 & 9.5\\
  \hline
  444.namd & 43.6 & 3.7 & 481.wrf & 33.6 & 11.1\\
  \hline
  437.leslie3d & 26.4 & 4.3 & 429.mcf &	83.74 & 11.5\\
  \hline
  403.gcc & 25.4 & 4.5 & 445.gobmk & 23.1 & 12.5\\
  \hline
  462.libquantum & 48.9 & 5.3 & 483.xalancbmk &	18.0 & 13.6\\
  \hline
  459.GemsFDTD & 21.6 & 5.5 & 435.gromacs & 31.4 & 15.6\\
  \hline
  470.lbm & 6.9 & 6.3 & 482.sphinx3 & 21 & 16.8\\
  \hline
  473.astar & 12.3 & 8.1 & 471.omnetpp & 26.2 & 17.5\\
  \hline
  456.hmmer & 17.9 & 8.1 & 465.tonto & 32.7 & 19.5\\
  \hline
\end{tabular}
}


==> applications-mise-model/tables/workload-stats.tex <==
\begin{footnotesize}
\begin{tabular}{|c|c|c||c|c|c||c|c|c||}
  \hline
  \textbf{Benchmark} & \textbf{LLC miss rate (MPKI)} & \textbf{IPC} & \textbf{Benchmark} & \textbf{LLC miss rate (MPKI)} & \textbf{IPC} & \textbf{Benchmark} & \textbf{LLC miss rate (MPKI)} & \textbf{IPC}\\
  \hline
  453.povray & 0.016 & 2.98 & 445.gobmk & 0.529 & 2.50 & 433.milc & 15.200 & 0.75\\
  \hline
  465.tonto & 0.022 & 2.98 & 435.gromacs & 0.975 & 2.32 & 483.xalancbmk & 17.988 & 0.64\\
  \hline
  454.calculix & 0.054 & 2.95 & 464.h264ref & 1.259 & 2.19 & 471.omnetpp & 18.879 & 0.73\\
  \hline
  400.perlbench & 0.077 & 2.95 & 456.hmmer & 2.830 & 1.65 & 459.GemsFDTD & 22.925 & 0.42\\
  \hline
  444.namd & 0.105 & 2.93 & 401.bzip2 & 4.061 & 1.77 & 470.lbm & 27.226 & 0.49\\
  \hline
  447.dealII & 0.115 & 2.90 & 436.cactusADM & 4.994 & 1.05 & 450.soplex & 27.341 & 0.51\\
  \hline
  481.wrf & 0.142 & 2.86 & 473.astar & 5.226 & 1.11 & 462.libquantum & 27.422 & 0.86\\
  \hline
  403.gcc & 0.224 & 2.81 & 482.sphinx3 & 13.151 & 0.72 & 429.mcf & 74.505 & 0.23\\
  \hline
  458.sjeng & 0.356 & 2.55 & 437.leslie3d & 14.250 & 0.80 & & &\\
  \hline
\end{tabular}
\end{footnotesize}


==> blacklisting/tables/interval-sensitivity.tex <==
\footnotesize{
%\begin{tabular}{|c|c|c|c|}
%  \hline
%   Epoch Length & 1000 & 10000 & 100000\\
%  \hline
%   Avg. Error (in \%) & 9.1 & 8.1 & 11.2\\
%  \hline
%  \hline
%  Interval Length & 1 mil & 5 mil & 10 mil\\
%  \hline
%  Avg. Error (in \%) & 64.1 & 8.1 & 9.6 \\
%  \hline
%\end{tabular}


\begin{tabular}{|c|c|c|c|c|c|}
  \hline
  {Interval Length} & 1000 & 10000 & 100000\\
  \hline 
  {Weighted Speedup} & 1.10 &  1.18 & 1.10\\
  \hline 
  {Maximum Slowdown} &  0.73 & 0.79 &  0.84\\
  \hline 
\end{tabular}
}


==> blacklisting/tables/shared-caches.tex <==
\begin{tabular}{|c|c|c|c|}
    \hline
    Metric & FRFCFS & TCM & BLISS\\
    \hline
    Weighted Speedup (Normalized) & 1 & 1.13 & 1.18\\
    \hline
    Maximum Slowdown (Normalized) & 1 & 0.99 & 0.75\\
    \hline
\end{tabular}


==> blacklisting/tables/threshold-sensitivity.tex <==
\footnotesize{
%\begin{tabular}{|c|c|c|c|}
%  \hline
%   Epoch Length & 1000 & 10000 & 100000\\
%  \hline
%   Avg. Error (in \%) & 9.1 & 8.1 & 11.2\\
%  \hline
%  \hline
%  Interval Length & 1 mil & 5 mil & 10 mil\\
%  \hline
%  Avg. Error (in \%) & 64.1 & 8.1 & 9.6 \\
%  \hline
%\end{tabular}

\begin{tabular}{|c|c|c|c|c|c|}
  \hline
  {Blacklisting Threshold} & 2 & 4 & 8 & 16\\
  \hline
  {Weighted Speedup} & 1.11 & 1.18 &  1.16 & 1.10\\
  \hline
  {Maximum Slowdown} & 0.75 & 0.79 &  0.89 & 0.75\\
  \hline 
\end{tabular}
}


==> mise/tables/perf-guarantees-stfm.tex <==
\footnotesize{
\begin{tabular}{|l|c|c|}
  \hline
  \textbf{Scenario} & \textbf{\# Workloads} & \textbf{\% Workloads} \\
  \hline
  Bound Met and Predicted Right & 1911 & 63.7\% \\
  \hline
  Bound Met and Predicted Wrong & 480 & 16\% \\
  \hline
  Bound Not Met and Predicted Right & 537 & 17.9\%  \\
  \hline
  Bound Not Met and Predicted Wrong & 72 & 2.4\%\\
  \hline
\end{tabular}
}  


==> mise/tables/perf-guarantees.tex <==
\footnotesize{
\begin{tabular}{|l|c|c|}
  \hline
  \textbf{Scenario} & \textbf{\# Workloads} & \textbf{\% Workloads} \\
  \hline
  Bound Met and Predicted Right & 2364 & 78.8\% \\
  \hline
  Bound Met and Predicted Wrong & 65 & 2.1\% \\
  \hline
  Bound Not Met and Predicted Right & 509 & 16.9\%  \\
  \hline
  Bound Not Met and Predicted Wrong & 62 & 2.2\%\\
  \hline
\end{tabular}
}  


==> mise/tables/workload-stats.tex <==
\begin{footnotesize}
\begin{tabular}{|c|c|c||c|c|c||c|c|c||}
  \hline
  \textbf{Benchmark} & \textbf{LLC miss rate (MPKI)} & \textbf{IPC} & \textbf{Benchmark} & \textbf{LLC miss rate (MPKI)} & \textbf{IPC} & \textbf{Benchmark} & \textbf{LLC miss rate (MPKI)} & \textbf{IPC}\\
  \hline
  453.povray & 0.016 & 2.98 & 445.gobmk & 0.529 & 2.50 & 433.milc & 15.200 & 0.75\\
  \hline
  465.tonto & 0.022 & 2.98 & 435.gromacs & 0.975 & 2.32 & 483.xalancbmk & 17.988 & 0.64\\
  \hline
  454.calculix & 0.054 & 2.95 & 464.h264ref & 1.259 & 2.19 & 471.omnetpp & 18.879 & 0.73\\
  \hline
  400.perlbench & 0.077 & 2.95 & 456.hmmer & 2.830 & 1.65 & 459.GemsFDTD & 22.925 & 0.42\\
  \hline
  444.namd & 0.105 & 2.93 & 401.bzip2 & 4.061 & 1.77 & 470.lbm & 27.226 & 0.49\\
  \hline
  447.dealII & 0.115 & 2.90 & 436.cactusADM & 4.994 & 1.05 & 450.soplex & 27.341 & 0.51\\
  \hline
  481.wrf & 0.142 & 2.86 & 473.astar & 5.226 & 1.11 & 462.libquantum & 27.422 & 0.86\\
  \hline
  403.gcc & 0.224 & 2.81 & 482.sphinx3 & 13.151 & 0.72 & 429.mcf & 74.505 & 0.23\\
  \hline
  458.sjeng & 0.356 & 2.55 & 437.leslie3d & 14.250 & 0.80 & & &\\
  \hline
\end{tabular}
\end{footnotesize}


==> mise/tables/workloads.tex <==
\footnotesize{
\begin{tabular}{|c|c|c|c|}
  \hline
  \textbf{Mix No.} & \textbf{Benchmark 1} & \textbf{Benchmark 2} & \textbf{Benchmark 3}\\
  \hline
  1 & sphinx3 & leslie3d & milc \\
  \hline
  2 & sjeng & gcc & perlbench \\
  \hline
  3 & tonto & povray & wrf \\
  \hline
  4 & perlbench & gcc & povray \\
  \hline
  5 & gcc & povray & leslie3d \\
  \hline
  6 & perlbench & namd & lbm \\
  \hline
  7 & hef & bzip2 & libquantum\\
  \hline
  8 & hmmer & lbm & omnetpp \\
  \hline
  9 & sjeng & libquantum & cactusADM \\
  \hline
  10 & namd & libquantum & mcf \\
  \hline
  11 & xalancbmk & mcf & astar \\
  \hline
  12 & mcf & libquantum & leslie3d \\
  \hline
\end{tabular}
}

